PairReranker: Pairwise Reranking for Natural Language Generation

Pre-trained language models have been successful in natural language generation (NLG) tasks. While various decoding methods have been employed, they often produce suboptimal results. We first present an empirical analysis of three NLG tasks: summarization, machine translation, and constrained text generation. We found that selecting the best output from the results of multiple decoding methods can significantly improve performance. To further improve reranking for NLG tasks, we proposed a novel method, \textsc{PairReranker}, which uses a single encoder and a pairwise loss function to jointly encode a source input and a pair of candidates and compare them. Experiments on three NLG tasks demonstrated the effectiveness and flexibility of \textsc{PairReranker}, showing strong results, compared with previous baselines. In addition, our \textsc{PairReranker} can generalize to significantly improve GPT-3 (text-davinci-003) results (e.g., 24.55\% on CommonGen and 11.35\% on WMT18 zh-en), even though our rerankers are not trained with any GPT-3 candidates.

==> sections/_alg.tex <==

\begin{algorithm}[t]
	\small 
    % \vspace{0.1em}
	\nonl \textbf{Input Data Clusters:}  {{$V_0, V_1, \dots, V_N$}} \\
% 	\vspace{0.1em}
	\nonl \textbf{Configuration Arguments}: $T, b, (\alpha, \beta, \gamma)$.  \\
% 	\vspace{0.1em}
	\nonl \textbf{Output}: A query stream $\{Q_1, Q_2, \dots, Q_T\}$
	%	\nonl {\scriptsize{/*~~*/}}
	
% 	\nonl{\textbf{Remarks}: $\Gamma_{n}(X)$ is a function to randomly sample $n$ unique elements from a set $X$.} \\ ~\\
	%	\comm{Add all tokens in to the token node set}
% 	\vspace{-1em}
	 
% 	\comm{Iterate each sampled distractor language $l_i$.} \\ 
	\ForEach{$t$ in $\operatorname{range}(1, T)$} { 
	   % $Q_t = [] $ ;
	   %\vspace{0.2em}
	    $b_u = \round{b * \alpha^{t-1}}$; $b_o = b -  b_u$ ; 
	    $b_o' = \round{b_o * \gamma} $ ; \\  
	   % \vspace{0.2em}
	    $c_t \sim P(c | c_{t-1}; \beta)$ \\
	   % \vspace{0.2em}
	    \comm{
	    The prob. of switching the major OOD data cluster is $1-\beta$, i.e.,
	    $P(c_t \neq  c_{t-1})=1-\beta$} \\
	   % \vspace{0.2em}
	    $V_{\neq c_t} = \bigcup_{\{k \in [1,N] | k \neq c_t\}} V_k$ \\ 
	   % \vspace{0.5em}
	    $Q_t {~\xleftarrow[]{}} \operatorname{sample}(V_0, b_u)$ \\ \comm{$V_0 \sim \mathcal{U}$; from upstream distribution} \\
		$Q_t \text{~+=~} \operatorname{sample}(V_{c_t}, b_o')$ \\ \comm{from the current major OOD data cluster} \\ 
		$Q_t \text{~+=~} \operatorname{sample}(V_{\neq c_t}, b_o-b_o')$ \\ \comm{from non-major data clusters}\\
% 		\comm{Add a distractor assertion as a candidate.}\\ 
% 		${C}$\text{.add}($M^{l_i}_j$)
        {$\operatorname{\textbf{assert}} ~|Q_t| = b$} 
        % \vspace{-1em}
	}
	\caption{\small{Sampling query streams with \textit{controllable non-stationarity} from multiple data clusters.}}\label{alg:cns}
\end{algorithm}



==> sections/_fig_curves.tex <==


\begin{figure*}[th!]
    % \vspace{-2em}
	\centering
% 	\hspace{-1.2em}
	\includegraphics[width=1\linewidth]{figures/curves.pdf}
	\caption{The curves of four key metrics over time of selected CMR methods in Table~\ref{tab:main}.  The $x$-axis is the time step.}
	\label{fig:curves}
\end{figure*}



==> sections/_fig_heatmap.tex <==


\begin{figure}[t]
% \vspace{-1em}
	\centering
% 	\hspace{-0.5em}
	\includegraphics[width=1\linewidth]{figures/heatmaps.pdf}
	\caption{  The differences between refined models produced by different CMR methods in terms of their predictions for the same inputs at two time spans (10-20 and 30-40). The darker cells have large discrepancy.}
	\label{fig:heatmap}
\end{figure}



==> sections/_fig_intro.tex <==


\begin{figure*}[t]
	\centering
% 	\hspace{-0.5em}
	\includegraphics[width=1\linewidth]{figures/cmr_formulation}
	\vspace{-1em}
	\caption{\small The continual model refinement (CMR) problem. We offline train a model $f_0$ and it may encounter many error cases $E_t$ when it is tested on a stream of query examples $Q_t$ over time which is drawn from ever-changing unseen distributions.
	A CMR method $g$ aims to fix the error cases over time by refining $f_{t}$ without catastrophic forgetting.   \vspace{-1em}}
	\label{fig:intro}
\end{figure*}
 

==> sections/_fig_methods.tex <==


\begin{figure*}[t]
% 	\centering
	\hspace{-0.5em}
	\includegraphics[width=1.03\linewidth]{figures/cmr_methods}
% 	\vspace{-1em}
	\caption{ The studied  methods for continual model refinement (Section~\ref{sec:methods}).  \vspace{-1em}}
	\label{fig:methods}
\end{figure*}
 

==> sections/_fig_metrics.tex <==


\begin{figure*}[t]
% 	\centering
	\hspace{-1em}
	\includegraphics[width=1.05\linewidth]{figures/cmr_metrics}
	\vspace{-1em}
	\caption{ The proposed five basic metrics for evaluating continual model refinement methods. \vspace{-1em}}
	\label{fig:metrics}
\end{figure*}
 

==> sections/_fig_stream.tex <==
 
\begin{figure*}[th!]
	\centering
% 	\hspace{-2em}
	\includegraphics[width=1\linewidth]{figures/submission_streams.pdf}
	\caption{\small The \textit{left} and \textit{middle} figures are two \textbf{query streams} of the QA task with different non-stationarity ($\beta=\{0.1, 0.5\}$) while sharing other arguments ($T$=50, $b$=64, $\alpha$=0.9, $\gamma$=0.8). 
	We use the blue color and `*' to denote the in-distribution data cluster (i.e., $V_0$), the percentage of which decay over time. 
	The distribution of incoming query examples dynamically shifts over time ---
	with larger $\beta$, adjacent episodes are more likely to share the same \textbf{major OOD clusters} which takes the $\gamma$ of the total OOD data.
	To encourage \textit{diversity}, the other $1-\gamma$ OOD examples are sampled from the remaining clusters.
	The \textit{right} figure is the \textbf{error stream} if we do not refine the upstream model (i.e., $f_t\equiv f_0$) and test it on the \textit{middle} query stream. } 
	\label{fig:submission_stream}
\end{figure*}

==> sections/_tab_main.tex <==

\begin{table*}[th!]
\centering
% \vspace{-1em}
% \hspace{-0.5em}
\scalebox{0.75}{
\begin{tabular}{r||c||cccc|c||cccc|c}
% \begin{tabular}{@{}lllllllll@{}}
\toprule
%  Question Answering $\rightarrow$ & - & \multicolumn{5}{c||}{\cellcolor{cyan!10}  } & \multicolumn{5}{c}{\cellcolor{blue!15} $()$ } \\ \midrule
  \textbf{Methods} $\downarrow$ \textbf{Metrics} $\rightarrow$ & \cellcolor{red!10} \AVG{EFR} & \cellcolor{blue!10} \AVG{UKR} & \cellcolor{blue!10} \AVG{OKR} & \cellcolor{blue!10} \AVG{CSR} & \cellcolor{blue!10} \AVG{KG} & \cellcolor{blue!10} \textbf{\AVG{OEC}} & \cellcolor{cyan!10} UKR\T & \cellcolor{cyan!10} OKR\T & \cellcolor{cyan!10} CSR\T & \cellcolor{cyan!10}KG\T & \cellcolor{cyan!10} \textbf{OEC\T} \\ \midrule 

 \rowcolor{gray!10}  Frozen Upstream ($f_t \equiv f_0$)  & 0.00  & 80.27 & 43.69 & 44.95 & 31.25 & 50.04 & 80.27 & 36.13 & 35.44 & 31.25 & 45.77 \\ \midrule
 {\color{gray}\ding{108}} \underline{Continual Fine-Tuning}   & 97.36 & 72.05 & 83.87 & 55.93 & 45.68 & 64.38 & 66.21 & 77.73 & 53.48 & 48.91 & 61.58 \\  \midrule 
{\color{brown}\ding{110}} \underline{Online L2Reg. }         & 97.18 & 73.47 & 85.37 & 57.27 & 47.12 & 65.81 & 71.09 & 83.59 & 54.50 & 51.17 & 65.09 \\
{\color[HTML]{7fc97f} \ding{115}} \underline{Online EWC}         & 97.49 & 73.38 & 86.09 & 56.17 & 47.34 & 65.75 & 68.55 & 85.74 & 53.67 & 53.28 & 65.31 \\ \midrule
{\color[HTML]{eb9634}\ding{58}} \underline{Exp. Replay (k=3)}    & 97.07 & 75.30 & 87.29 & 56.02 & 47.61 & 66.55 & 72.46 & 87.30 & 54.08 & 52.66 & 66.63 \\
Experience Replay (k=1)    & 96.72 & 78.91 & 89.38 & 57.80 & 47.17 & 68.31 & 78.13 & 86.52 & 55.33 & 52.73 & 68.18 \\ \midrule
% Dense Retrieval (k=1)      & 97.29 & 78.04 & 88.18 & 57.66 & 47.39 & 67.82 & 77.73 & 84.96 & 55.50 & 51.80 & 67.50 \\ \midrule
{\color[HTML]{c334eb} \ding{117}} \underline{MaxLoss (k=3,c=256)}      & 97.43 & 75.43 & 86.89 & 57.14 & 46.70 & 66.54 & 75.00 & 84.77 & 55.11 & 51.33 & 66.55 \\
MaxLoss (k=1,c=256)      & 96.54 & 78.16 & 89.86 & 57.78 & 46.63 & 68.11 & 77.54 & 89.26 & 55.47 & 50.94 & 68.30 \\
MaxLoss (k=1,c=512)       & 97.41 & 75.57 & 87.09 & 56.80 & 46.45 & 66.48 & 77.54 & 89.65 & 55.88 & 52.81 & 68.97 \\
MaxLoss (k=1,c=1024)   & 96.63 & 77.61 & 89.82 & 58.13 & 47.10 & 68.17 & 80.66 & 91.02 & 55.88 & 50.78 & 69.59 \\
 \midrule
% $\rhd$
{\color[HTML]{386cb0}$\righttriangle$} \underline{MIR (k=3,c=256)} & 97.08 & 75.92 & 87.13 & 56.91 & 47.22 & 66.79 & 75.78 & 87.50 & 54.53 & 51.80 & 67.40 \\
MIR (k=1,c=256)     & 96.59 & 77.84 & 89.77 & 58.35 & 47.28 & 68.31 & 79.49 & 90.43 & 55.91 & 51.25 & 69.27 \\
MIR (k=1,c=512)     & 96.96 & 77.86 & 89.41 & 58.13 & 46.40 & 67.95 & 79.69 & 89.45 & 55.50 & 50.08 & 68.68 \\
MIR (k=1,c=1024) & 96.71&	77.47&	87.83&	57.98&	46.87&	67.54&	78.13&	87.89&	55.73&	50.70&	68.11 \\ \midrule
{MIR(1,256)}+OnlineL2Reg          & 96.15&	79.10&	90.41&	59.80&	47.90&	69.30 & 79.49 & 90.04 & 57.45 & 52.66 & 69.91 \\
\midrule
 \rowcolor{gray!20}   Offline Refining ($f_0 \rightarrow f_T$)    & \textit{95.62} &	- & - & - &	- & - & \textit{83.78} & 	\textit{93.75} & \textit{93.81} &	\textit{56.17} &	\textit{81.88 }
%  0.837890625,0.9375,0.938125,0.56171875,0.81880859375
 \\
\bottomrule


\end{tabular}
}
\caption{\small Results (\%) in multiple metrics: \textbf{EFR}=Error-Fixing Rate; \textbf{UKR/OKR}=Upstream/Online Knowledge Retention; \textbf{CSR}=Cumulative Success Rate; \textbf{KG}=Knowledge Generalization. \textbf{OEC} is the average of the last four. Column names with bars are the average of all periods. The ones with `\T' are the scores at the final step.
The underlined methods are matched with the legends in Figure~\ref{fig:curves}. $k$ is the replay interval (the smaller the more frequent), and $c$ is the size of the candidate pool.  }
\label{tab:main}
\end{table*}


\begin{table}[htb]
\begin{center}
    \scalebox{0.75}{
    \begin{tabular}{c c c c c}
        \hline
         Decoding method & \# Candidates & R-1 & R-2 & R-L  \\
        \hline
        Top beam & 1 & 44.22 & 21.48 & 41.21\\
        \hline
         Beam Search & 15 & 51.06 & 27.74 & 48.05 \\
         Diverse Beam Search & 15 & 54.30 & 30.02 & 51.33\\
         Top-k sampling & 15 & 52.32 & 27.74 & 49.19 \\
         Top-p sampling & 15 & 53.51 & 28.83 & 50.40 \\
         \hdashline
         Adding all & 57.70 & 33.75 & 57.42 \\
        \hline
    \end{tabular}}
    \caption{\label{oracle_gap_cnndm} Oracle selection performance on CNN/Daily Mail using finetuned PEGASUS-large. Same as \citet{Ravaut2022SummaRerankerAM}}
\end{center}
\end{table}













==> sections/_tab_settings.tex <==

\begin{table}[t]
% \vspace{-1em}
\centering
% \hspace{-0.3em}
\scalebox{0.74}{
\begin{tabular}{r||ccccc}
\toprule 
 \textbf{Stream Dynamics}                              & \textbf{CFT}     & \textbf{EWC}   & \textbf{ER}      & \textbf{MxLs}   & \textbf{MIR}   \\ \toprule
 
% &  { $\\alpha$=0.9, $\\beta$=0.5, $\\gamma$=0.8} & 61.58  & 65.31  & 66.11  & 68.27  & 67.52   \\ \midrule
% &  $\\alpha$=0.9, $\\beta$=\textbf{0.1}, $\\gamma$=0.8 & 62.73  & 63.06  & 67.05  & 66.57  & 65.55  \\
% &  $\\alpha$=0.9, $\\beta$=\textbf{0.9}, $\\gamma$=0.8 & 64.58  & 65.32  & 67.50  & 67.23  & 67.22  \\  \midrule
% &  $\\alpha$=0.9, $\\beta$=0.5, $\\gamma$=\textbf{0.2} & 64.53  & 64.67  & 66.54  & 67.57  & 66.60   \\  
% &  $\\alpha$=0.9, $\\beta$=0.5, $\\gamma$=\textbf{0.5} & 63.86  & 64.62  & 66.02  & 64.75  & 65.85   \\\midrule
% &  $\\alpha$=\textbf{0.9}, $\\beta$=0.5, $\\gamma$=0.6 & 64.42  & 63.27  & 66.20  & 67.65  & 66.50  \\ 
 
%  $\alpha$=0.9, $\beta$=0.5, $\gamma$=0.8 & 61.6  & 65.3  & 66.1  & 68.3   & 67.5  \\ \midrule
%  $\alpha$=\textbf{0.1}, $\beta$=0.5, $\gamma$=0.8 & 64.5  & 64.7  & 66.5  & 67.6   & 66.6  \\ \midrule
%  $\alpha$=0.9, $\beta$=\textbf{0.1}, $\gamma$=0.8 & 62.7  & 63.1  & 67.1  & 66.6   & 65.6  \\
%  $\alpha$=0.9, $\beta$=\textbf{0.9}, $\gamma$=0.8 & 64.6  & 65.3  & 67.5  & 67.2   & 67.2  \\
%  \midrule
%  $\alpha$=0.9, $\beta$=0.5, $\gamma$=\textbf{0.2} & 63.9  & 64.6  & 66.0  & 64.8   & 65.8  \\
%  $\alpha$=0.9, $\beta$=0.5, $\gamma$=\textbf{0.5} & 64.4  & 63.3  & 66.2  & 67.6   & 66.5  \\
\rowcolor{gray!20} 
 $\alpha$=0.9, $\beta$=0.5, $\gamma$=0.8 & 15.81&	19.54&	20.86&	20.78&	21.63   \\ \midrule
%  $\alpha$=\textbf{0.1}, $\beta$=0.5, $\gamma$=0.8 & 17.29&	17.62&	21.62&	21.14&	20.12\\ \midrule
 $\alpha$=0.9, $\beta$=\textbf{0.1}, $\gamma$=0.8 & 23.40&	24.14&	26.32&	26.05&	26.04 \\
 $\alpha$=0.9, $\beta$=\textbf{0.9}, $\gamma$=0.8 & 18.61&	19.38&	20.78&	19.51&	20.60 \\
 \midrule
 $\alpha$=0.9, $\beta$=0.5, $\gamma$=\textbf{0.5} & 19.97&	20.10&	21.97&	23.01&	22.04 \\
 $\alpha$=0.9, $\beta$=0.5, $\gamma$=\textbf{0.2} & 17.37&	16.22&	19.15&	20.60&	19.45 \\
 \bottomrule


\end{tabular} 
}
\caption{\small The \textbf{\textit{gain}} of OEC\T over the \textit{Frozen Upstream} baseline for each method under different stream dynamics. \vspace{-0.5em}}
\label{tab:settings}
\end{table}

